The Rizzeta Stone: Adopting Gen-$\alpha$ Colloquial Language to Improve Scientific Paper Rizz and Aura from a Skibidi Perspective

The field of astronomy evolves rapidly, and it is essential to keep up with these changes in order to effectively communicate with the broader community. However, communication itself also changes as new words, phrases, and slang terms enter the common vernacular. This is especially true for the current youngest generations, who are capable of efficiently communicating via the Internet. In order to maintain effective communication, we explore the possibility of expanding the language used in scientific communication to include recently coined slang. This attempt at outreach, while potentially very difficult, could provide a means to expand the field and capture the attention of early-career scientists, improving retention within the field. However, our results indicate that, while possible, this method of communication is, like, probably not really worth it, no cap.

==> Glossary.tex <==
aura -

ohio -

rizz- Short for "charisma", typically used in the same sorts of contexts, but more casually. Can also be used as a verb to mean something to the effect of "applying charisma", e.g. "He is rizzing up his boss in hopes of a raise"

skibidi -

==> SlangTable.tex <==
\begin{table*}[]
    \centering
    \begin{tabular}{cc|l|l|l}
     &Term & Definition & Sample Sentence & Usage Notes \\
    \hline\hline
    \multirow{14}{*}{Positive}   &Aura {\it n.} & A likeable demeanor & {\it``Bro's got {\bf aura}, you see } & \\
    & & &{\it everybody laughing around him?''} &\\
    & Gucci {\it adj.} &Good; in good standing  &{\it ``Don't worry about it man,}  &Can be used to describe \\
    & & &{\it we're {\bf Gucci}''} &anything good but is more \\
    & & & & frequently used to express  \\
    & & & & being okay, see e.g. \\
    & & & &``I'm good/I'm Gucci'' \\
    & Gyatt {\it n.} & An attractive buttocks &{\it ``Did you see that {\bf gyatt?}} &\\
    & & & {\it [REDACTED]''} & \\
    & Rizz {\it n.}& The ability to sway others, &{\it ``She's got unimaginable {\bf rizz};} &Often used in a similar \\
    & & particularly in the context of &{\it she came out of the} &manner to ``aura'' (above) \\
    & & courtship and dating.&{\it bar with ten phone numbers.''} &but is frequently turned into a \\
    & & Derived from charisma. & & \\
    & & & &  verb e.g. rizz/ing to describe\\
    & & & &  the act of swaying others\\
    
    \hline
    \multirow{14}{*}{Neutral} & Chat {\it n.} & An (often intangible) group  &{\it ``Chat, does this look right?} &Typically used to address an \\
    & &of people & &audience (real or imaginary) as  \\
    & & & & a means of voicing ideas or   \\
    & & & &receiving feedback  \\
    & Cook {\it v.} &To continue to act towards a& {\it ``He's almost got it,} &While ``cook'' is typically used\\
    &  &strictly positive or negative &{\it let him {\bf cook!}''} & to describe action toward\\
    &&outcome &&a positive outcome, it is frequently \\
    &&&&used ironically. ``Cooked {\it adj.}''  \\
    &&&&usually  means something like\\
    &&&& ``defeated'' or ``finished''\\
    & High-Key {\it adv.} & Without subtlety &{\it ``I'm {\bf high-key} excited } &While its antonym ``low-key''  \\
    &&&{\it for the concert tonight!''}& means ``subtley'', ``high-key'' is   \\
    &&&&typically used as an intensifier\\
    & Skibidi {\it adj.} &``Good" or positive&{\it ''{My boyfriend bought me my }} & From popular YouTube Series \\
    && & \it{favorite flowers, he is so \bf skibidi!}" &Skibidi Toilet, the word has \\
    && & &since separated from the series\\
    \hline
    \multirow{15}{*}{Negative} & Brainrot {\it n.} & The resultant state of an  &{\it ``Carol really needs to lay off } &While often used derisively,  \\
    & &overuse of social media,  & {\it TikTok before that {\bf brainrot} gets}&it can also describe the\\
    & &typically presenting as having a &{\it out of hand''} &genre of humor that  \\
    & &short attention span and    & &utilizes ``brainrot'' slang \\
    & &a vocabulary comprised mainly& &\\
    & &  of recent internet slang & &\\
    & Cap {\it n.} & Lie; un-truth &{\it ``George said they're coming to the} &Often phrased ``No cap'' to \\
    & & & {\it party, but that's {\bf cap}.''} &indicate honesty \\
    & Opp {\it n.} & A person opposed to someone &{\it ``Frankie's {\bf opps} are praying} &Not typically used to \\
    &&&{\it praying on his downfall.''}&refer to a specific person,\\
    &&&& but instead refers to a general\\
    &&&& force of opposition\\
    & Ohio {\it adj.} & Weird; Strange & & \\
    & Sus {\it adj.} &Untrustworthy &{\it ``That guy in the trenchcoat behind} & \\
    & & &{\it the hardware store is real {\bf sus}.''} &\\
    \hline
    
    
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table*}

==> SlangTable_Rizzed.tex <==
\begin{table*}
\center
%\setlength\extrarowheight{-1pt}
\begin{tabular}{p{3cm} | p{4cm}| p{4cm} | p{4cm} } 
%\center
Term & Definition & Sample Sentence & Usage Notes \\
\hline
\hline
Aura \textit{n.} & A likeable/imposing demeanor, often determined just by appearance & \textit{``Bro has such \textbf{aura}, you see everyboday laughing around him?"} & ``Aura Farming" is a common usage, attempting to look cool frequently without actually doing anything \\
GOAT \textit{n.} & Acronym for ``Greatest of all Time" & \textit{``Michael Jordan is the \textbf{GOAT} of basketball."} & \\
Gucci \textit{adj.} &  Good; in good standing & \textit{``Don't worry about paying me back man, we're \textbf{Gucci}"} & Originates from the high-end clothing retailer.\\
Gyatt \textit{n.} & An attractive buttocks & \textit{``Did you see that \textbf{gyatt}? [REDACTED]"} & Not suitable for serious academic use.\\
King/Queen \textit{n.} & Gendered terms signifying high status & ``\textbf{king}" & Also used as an adjective to describe activities befitting such a person, usually accompanied with explicatives. \\
Rizz \textit{n.} & Derived from \textit{charisma}, an ability to sway others, particularly in the context of courtship and dating & \textit{``She's got unimaginable \textbf{rizz}; she came out of the bar with ten phone numbers."} & Also applicable as a verb, e.g. rizz/ing to describe the act of swaying others\\
Skibidi \textit{adj.} & General term meaning ``Good" or something positive, occasionally used as a filler word. & \textit{``My boyfriend bought me my favorite flowers, he is so \textbf{skibidi}!"} & From popular YouTube series Skibidi Toilet, the word has since decoupled from the series.\\
\hline
Chat \textit{n.} & A group of omniscient observers & \textit{``Can you believe this \textbf{chat}?"} & Originated from video game streamers referring to their audience, often used to imitate them. \\
Cook \textit{v.} & To continue to ac towards a strictly positive or negative outcome & \textit{``He's almost got it, let him \textbf{cook!}} & While ``cook" is typically used to describe action toward a positive outcome, to be ``cooked" \textit{adj.} implies the opposite, i.e. to be ``defeated" or ``finished".\\
High-Key \textit{adv.} & Without subtlety & \textit{``I'm \textbf{high-key} excited for the concert tonight!"} & While its antonym ``low-key" means ``subtlety", high-key is typically used as an intensifier. \\
Mad \textit{adj.} & A lot of; a great deal of something & \textit{`` Lizzy has \textbf{mad} skills when it comes to understanding quantum computers!} & \\
On-God & Truthful, particularly when a claim is faced with doubt & \textit{``\textbf{On-God}, I caught an alligator two feet long in my backyard last week!"} & \\
Out of Pocket \textit{adj.}  & Random or unexpected, but usually in a lighthearted manner & \textit{``Sarah's comment on bird mating habits was very \textbf{out of pocket} given we were discussing neutron stars, but it was pretty funny."} & \\
\hline
Brainrot \textit{n.} & The resultant state of an overuse of social media, typically presenting as having a short attention span and a vocabulary comprised mainly of internet slang & \textit{``Carol needs to lay off TikTok, her \textbf{brainrot} has gotten so bad I can hardly understand her.} & While often used derisively, it can also describe the genre of humor that utilizes `brainrot' slang. \\
Cap \textit{n.} & Lie; an un-truth & \textit{"George said they're coming to the party, but that's \textbf{cap}."} & Often phrased ``No Cap" to indicate honesty. \\
Opp \textit{n.} & A person opposed to someone; an enemy & \textit{``Frankie's \textbf{opps} are praying on his downfall."} & Typically used to refer to a general force of opposition, not a single person.\\
Ohio \textit{adj.} & Weird; Strange & \textit{"I feel sick to my stomach, that lunch was definately made in \textbf{Ohio}."} &  \\
Sus \textit{adj.} & Untrustworthy or suspicious & \textit{``That guy in the trenchcoat behind the hardware store is real \textbf{sus}.} &  \\
Unc \textit{n.} & Short for "uncle", refers to an older person than the speaker, although typically with a negative connotation implied. & \textit{``Look at \textbf{unc}! Despite his knee surgery, he does still have some skill left in him."} & \\
\end{tabular}
%\end{center}
\end{table*}

